Equivalence of Meson Scattering Amplitudes in Strong Coupling Lattice and Flat Space String Theory

We consider meson scattering in the framework of the lattice strong coupling expansion. In particular we derive an expression for the 4-point function of meson operators in the planar limit of scalar Chromodynamics. Interestingly, in the naive continuum limit the expression coincides with an independently known result, that of the worldline formalism. Moreover, it was argued by Makeenko and Olesen that (assuming confinement) the resulting scattering amplitude in momentum space is the celebrated expression proposed by Veneziano several decades ago. This motivates us to also use holography in order to argue that the continuum expression for the scattering amplitude is related to the result obtained from flat space string theory. Our results hint that at strong coupling and large-$N_c$ the naive continuum limit of the lattice formalism can be related to a flat space string theory.

==> 04-lattice2.tex <==
\section{Back to the Lattice: Strong Coupling Expansion}
